Probabilistic Safety Constraints for Learned High Relative Degree System Dynamics

This paper focuses on learning a model of system dynamics online while satisfying safety constraints.Our motivation is to avoid offline system identification or hand-specified dynamics models and allowa system to safely and autonomously estimate and adapt its own model during online operation.Given streaming observations of the system state, we use Bayesian learning to obtain a distributionover the system dynamics. In turn, the distribution is used to optimize the system behavior andensure safety with high probability, by specifying a chance constraint over a control barrier function.

==> old/abstract-1.tex <==
This paper studies safe exploration in a system with unknown system dynamics.
A common approach to guarantee safety is Control Barrier Functions (CBF).
CBFs can be intuitively understood as Lyapunov functions applied to the safe region instead of an equilibrium point.
We use Bayesian learning algorithms to estimate a distribution over the dynamics, leading to a distribution over CBF.
We then formulate the control problem as a Quadratic Program with a chance constraint over CBFs.
In our experiments, we compare the safety performance of different Bayesian learning algorithms versus the number of samples and the variance of the prior distribution.

==> old/evaluation-known-dynamics.tex <==
Consider a pendulum system with state Let $\bfx=[\theta,\omega]^\top$, and
system dynamics,
\begin{align}
\dot{\bfx}=
\underbrace{\begin{bmatrix}
\omega
\\
-\frac{g}{l} \sin \theta
\end{bmatrix}}_{f(\bfx)}
+ 
  \underbrace{
\begin{bmatrix}
0
\\
\frac{1}{ml}  
\end{bmatrix}
    }_{g(\bfx)}
\bfu.
\end{align}
The notion of Lyapunov
function has played a predominant role in the investigation
of liveness properties~\cite{ames2014rapidly}. In fact, as it shown in~\cite{cbf,ames2016control,cbf_car}, given the Control Lyapunov Function (CLF) $V$, the following optimization-based controller 
\begin{align}
\label{QP-CLF-CBF234wew1}
\min_{\bfu_{k} \in \mathcal{U}} \;\;& \bfu_kQ\bfu_k
%\\
& \text{s.t.}~~ &\mbox{CBC}_k \ge 0,
%\\
&\mbox{CLC}_k &\le 0.
\end{align}
is constraint to both safety and liveness propersties, where
\begin{align}
    \mbox{CLC}_k=\mathcal{L}_{f} V(\bfx_k)+\mathcal{L}_{g}V(\bfx_k) \bfu_k+c V(\bfx_k),
\end{align}
for some constant $c >0$, is the Control Lyapunov Condition. 



Define the  control Lyapunov function
\begin{align}
    V(\bfx)=\frac{1}{2}ml^2\omega^2+mgl(1-\cos{\theta})
\end{align}
Note that $V$ is the non-negative function which is only zero at $\theta=\omega=0$, where $\theta \in [0,2\pi]$.
Thus,
%
\begin{align}
    \nabla_\bfx V(\bfx) &= [mgl \sin(\theta),ml^2\omega]^\top,
  \\
  \mathcal{L}_{f} V(\bfx) &= \grad_\bfx V(\bfx)^\top f(\bfx) = 0
  \\
  \mathcal{L}_{g} V(\bfx) &= \grad_\bfx V(\bfx)^\top g(\bfx) =[g\sin(\theta), l\omega].
\end{align}
%

We define the Exponential CBF as to avoid the unsafe red region
$[\theta_c - \Delta_c, \theta_c + \Delta_c]$ as shown in Figure~\ref{fig:CPS}.
%
\begin{align}
h(\bfx) = \cos(\Delta_{col}) - \cos(\theta - \theta_c).
\end{align}%
% 
The Lie derivatives of CBF are given by
%
\begin{align}
\grad_\bfx h(\bfx) &= [\sin(\theta - \theta_c), 0]^\top
  \\
  \Lie_f h(\bfx) &= \grad_\bfx h(\bfx)^\top f(\bfx)
                   = \omega\sin(\theta - \theta_c)
  \\
  \Lie_gh(\bfx) &= \grad_\bfx h(\bfx)^\top g(\bfx)
                   = 0
  \\
  \grad_\bfx \Lie_fh(\bfx) &= [-\omega\cos(\theta - \theta_c), \sin(\theta - \theta_c)]^\top
  \\
  \Lie_f^2 h(\bfx) &= \grad_\bfx \Lie_fh(\bfx)^\top f(\bfx)
  \\
                   &= [f(\bfx)^\top H_{xx}h(\bfx) + \grad_\bfx h(\bfx)^\top J_xf(\bfx) ] f(\bfx)
  \\
                   &= -\omega^2\cos(\theta - \theta_c) - \frac{g}{l}\sin(\theta - \theta_c)\sin(\theta)
  \\
  \Lie_g \Lie_f h(\bfx) &= \grad_\bfx \Lie_f h(\bfx)^\top g(\bfx)
  \\
                   &= [f(\bfx)^\top H_{xx}h(\bfx) + \grad_\bfx h(\bfx)^\top J_xf(\bfx) ] g(\bfx)
  \\
                   &= \frac{1}{ml}\sin(\theta - \theta_c)
\end{align}%
% 
The control barrier condition is then given by
%
\begin{align}
  \Lie_f^2 h(\bfx) + \Lie_g \Lie_f h(\bfx) \bfu
  + K_\alpha  \begin{bmatrix} h(\bfx) \\ \Lie_f h(\bfx) \end{bmatrix}  \ge 0,
\end{align}%
% 
where $K_\alpha = [1, 1]$ is chosen to satisfy Theorem 8 in \cite{cbf}.



\paragraph{Parameters}
$\theta(0)=150$, $\omega(0)=-0.01$, $\tau=0.01$, $m=1$, $g=10$, $l=1$.

$\theta_c=45$ $\Delta_{col}=22.5$


% \begin{figure*}[t]
% \centering
% \begin{tabular}{c c c}
%     \includegraphics[width=53mm]{fig/Figure1.pdf} &
%     \includegraphics[width=53mm]{fig/Figure2.pdf} &
%     \includegraphics[width=53mm]{fig/Figure3.pdf} 
% \end{tabular}
% \caption{Results}
% \label{simres}
% \end{figure*}

==> old/gaussian-process-attempt.tex <==
\section{Previous attempts at Gaussian distribution}
We note that $\ctrlaff \in
\R^{(1+m) \times 1}$.
Sampled at time $t$, the output of $\dynAff(\state_t) \in \R^{(1+m)
  \times n}$ gets mapped to
$\stdt_{t} := \frac{\state_{(t+1)} - \state_{t}}{\dt}$ as
$\stdt_{t} = \Y_t^\top\ctrlaff_t$.
Since the affine mapping is deterministic and without noise, we can solve the
linear system $\ctrlaff_t^\top \Y_t = \stdt_t^\top$ for possible $\Y_t$.
Using pseudo-inverse all possible solutions for $\Y_t$ are parameterized by
$\W_t$ as
%
\begin{align}
  \Y_t = \frac{\ctrlaff_t}{\|\ctrlaff_t\|^2_2} \stdt_t^\top
  + \left(I - \frac{\ctrlaff_t \ctrlaff_t^\top}{\|\ctrlaff_t\|^2_2}\right)\W_t,
\end{align}%
% 
where $\frac{\ctrlaff_t}{\|\ctrlaff_t\|^2_2}$ is the pseudo-inverse of
$\ctrlaff_t^\top$.
Let $\V_t := \left(I - \frac{\ctrlaff_t
    \ctrlaff_t^\top}{\|\ctrlaff_t\|^2_2}\right)$,
$\M(\state_t) :=  \frac{\ctrlaff_t^\top}{\|\ctrlaff_t\|^2_2}\stdt_t^\top$ and $\W_t$ be
generated by a stationary function of $\state_t$ as $\W_t = \mH(\state_t)$, then
%
\begin{align}
  \dynAff(\state_t) = \Y_t = \M(\state_t) +  \V_t\W_t = \M(\state_t, \ctrlaff_t) + \V_t\mH(\state_t)
\end{align}%
% 

Note that $\bY_t$ and $\V_t$ are deterministic functions $\stdt_t$ and
$\ctrlaff_t$, leaving only $\W_t = \mH(\state_t)$ to be the random matrix to be
chosen by $\state_t$. Since $\dynAff$ is a linearly related to $\mH$, $\mH$ is
also a Gaussian process. Let
%
\begin{align}
\mH \sim \GP(0, \kH).
\end{align}%
% 
where the 4-D kernel function $\kH(\state, \state') \in \R^{(1+m)\times n \times
n \times (1+m)}$ can be factorized into the covariance due to $\state$,
$\knl(\state, \state')$ and the
covariance between the output dimensions $\KH_{i,j,k,l}$,

%
\begin{align}
[\kH(\state, \state')]_{i,j,k,l} = \KH_{i,j,k,l} k(\state, \state').
\end{align}%
% 

The corresponding gaussian process for $\dynAff$ is,
%
\begin{align}
\dynAff &\sim \GP(0, \kDA),
  \\
\text{ where }[\kDA(\state, \state')]_{i,j,k,l} &= \sum_{o,p} \V_t[i,o] \KH_{o,j,k,p}\V_t^\top[p,j] \knl(\state, \state'),
\end{align}%
% 

Let $\dynAff(\state)$ be a Gaussian Process with mean function as
$\bDynAff(\state) = \smallbmat{\bDynSt(\state)& \bDynCt(\state)}$ and kernel
function as separable
% $\covf(\dynAff(\state), \dynAff(\state'))^{(i,j)} = \bKF^{(i,j)}\bKx(\state, \state')$.
Let us assume that we have a dataset
$\Data = \{\{\dSt_{t\dt,k},
\state_{t\dt,k}, \ctrlaff_{t\dt,k}\}_{t=1}^T\}_{k=1}^N$, where $\dt$ is the
discretization of the time and  is the discrete approximation of state derivative at $\dt$ .
Linear scaling of $\dynAff(\state)$ to $\dynAff(\state)\ctrlaff $ is also a
Gaussian process with mean $\dynAff(\state)\ctrlaff$ and covariance 
%$\covf(\dynAff(\state)\ctrlaff, \dynAff(\state')\ctrlaff')^{(i,j)} = \bKFu^{(i,j)}(\ctrlaff)\bKx(\state, \state')$.
The relationship between the affine kernel is determined by reshaping the $\bKF$
to a 4-D tensor $\bKF \in \R^{(1+m)\times n  \times n \times (1+m)}$ and then taking the dot product $\bKFu^{(i, j)}(\ctrlaff) = \sum_{k=1,l=1}^{(1+m),(1+m)}
\ctrlaff^{(k)}\bKF^{(k, i, j, l)} \ctrlaff^{(l)}$.

%
% \begin{align}
%   p(\dynAff(\StDat)) &= \N(\bDynAff(\StDat), \bKF \otimes \bKx(\StDat, \StDat))
%   \\
%   p(\dynAff(\StDat)\CtDat) &= \N(
%                              \bDynAff(\StDat)\CtDat,
%                              \underbrace{
%                              \CtDat^T[\bKF \otimes \bKx(\StDat, \StDat)]\CtDat
% }_{\bKFux(\CtDat, \StDat, \StDat, \CtDat)}
%                              )
% \end{align}
%
where $\StDat \in \R^{d \times n}$ is the state data matrix with $d$ data
samples and $n$ features. Similarly, $\dynAff(\StDat) \in \R^{d \times n \times (1+m)}$,
and $\CtDat \in \R^{d \times (1+m)}$. In the data matrix context, we assume that
matrix multiplication is over each data sample i.e.
$[\dynAff(\StDat)\CtDat]^{(k,:)} = \dynAff(\StDat^{(k,:)})\CtDat^{(k,:)}$.
Hence $\dynAff(\StDat)\CtDat \in \R^{d \times n}$. Similarly the data covariance
is assumed to matrix multiple on per data sample basis,
%$[\CtDat^T[\bKF \otimes \bKx(\StDat, \StDat)]\CtDat]^{(k,:)} = \CtDat^{(k,:)T}[\bKF \otimes \bKx(\StDat, \StDat)]^{(k,k)}\CtDat^{(k,:)}$.

%
\begin{multline}
  p(\dynAff(\state_*)\ctrlaff_*| \StDtDat, \state_*,\ctrlaff_*,\StDat,\CtDat)
  \\= \N(
  \bKFux(\ctrlaff_*, \state_*, \StDat, \CtDat)
  \bKFux(\CtDat, \StDat, \StDat, \CtDat)^{-1}
  \StDtDat,
  \\
  \bKFux(\ctrlaff_*, \state_*, \StDat, \CtDat)
  \bKFux(\CtDat, \StDat, \StDat, \CtDat)^{-1}
  \bKFux(\CtDat, \StDat, \state_*, \ctrlaff_*)
  )
\end{multline}%
% 


%
\begin{multline}
  p(\dynAff(\state_*)| \StDtDat \CtDat^{-\dagger}, \state_*,\StDat)
  \\= \N(
  \bKFx(\state_*, \StDat)
  \bKFx(\StDat, \StDat)^{-1}
  \StDtDat \CtDat^{-\dagger},
  \\
  \bKFx(\state_*, \StDat)
  \bKFx(\StDat, \StDat)^{-1}
  \bKFx(\StDat, \state_*)
  )
\end{multline}%
% 

==> old/trash.tex <==
Expanding the gradient of $\Lie_fh(\bfx)$, we get:
\begin{align}
  \grad \Lie_f h(\bfx) &= \grad [\grad h(\bfx)^\top f(\bfx)]
                              = H_{xx} h(\bfx)f(\bfx) + J_x^\top f(\bfx) \grad h(\bfx)
                              \quad (\text{See~\ref{proof:grad-of-lie-h}}).
                              \label{eq:grad-of-lie-h}
\end{align}
%
Here the first term $H_{xx} h(\bfx)f(\bfx)$ is simply a matrix multiplication to
a Gaussian process resulting in again a Vector-valued Gaussian process with mean and variance,
%
\begin{align}
  \E[H_{xx} h(\bfx)(\barf + \tdf)(\bfx)] &= h(\bfx)(\barf + \mutdf)(\bfx)
  \\
  \Cov[H_{xx} h(\bfx)(\barf + \tdf)(\bfx)] &= \ktdf(\bfx, \bfx') H_{xx} h(\bfx') K^f H_{xx} h(\bfx')^\top
\end{align}%
% 

The distribution of $J_x^\top f(\bfx) \grad h(\bfx)$ needs to compute the
derivative of a Vector-valued Gaussian Process. Since differentiation is a
linear operation, the result is again a Gaussian Process. To compute it, we need
the following Lemmas.


Using these Lemmas, we can compute the mean and variance of $J_\bfx^\top f(\bfx)
\grad h(\bfx)$,
%
\begin{align}
  \E[J_\bfx^\top f(\bfx)\grad h(\bfx)] &= J^\top_\bfx \barf(\bfx)\grad h(\bfx)
                            + \vect^{-1}_{n \times n}\left(
                            \left[[J_{\bfx_*}^\top \bfkx \bfKX] \otimes I_{n \times n}\right] \bfY\right)^\top
\grad h(\bfx)
  \\
  \Var(J_\bfx^\top f(\bfx)\grad h(\bfx))
  &= 
\left[ H_{xx} k(\bfx_*, \bfx'_*)
    - J_{\bfx_*}^\top \bfkx\bfKX J_{\bfx_*}\bfkxp \right] \grad h(\bfx)^\top K^f \grad h(\bfx),
\end{align}%
% 
where $\vect^{-1}_{n \times l} : \R^{nl}  \to \R^{n \times l}$ converts a vector
to a matrix by wrapping it along the columns.


%
\begin{align}
  \E[\grad_{\bfx} \Lie_f h(\bfx)]
  &= \grad \Lie_{\barf} h(\bfx)
    + H_{xx}h(\bfx) [\bfkx^\top \bfKX] \otimes I_{n \times n}] \bfY
    \nonumber
  \\
    & \qquad + \vect^{-1}_{n \times n}\left(
  [J_\bfx^\top\bfkx \bfKX] \otimes I_{n \times n}] \bfY \right)^\top \grad h(\bfx)
  \\
  \Var(\grad\Lie_fh(\bfx))
  &= [k(\bfx, \bfx') - \bfkx^\top\bfKX\bfkx] H_{xx}h(\bfx) K^f H_{xx} h(\bfx')^\top
    \nonumber
    \\
    &\quad +  \left[ H_{xx} k(\bfx_*, \bfx'_*)
    - J_{\bfx_*}^\top \bfkx\bfKX J_{\bfx_*}\bfkxp \right] \grad h(\bfx)^\top K^f \grad h(\bfx)
\end{align}%
% 


%%%%%%%%%%%%%%%%%%%%% Vector variate Gaussian processes


\begin{lemma}[Vector-variate Gaussian Processes]
  \label{thm:multi-variate-gp}
Let the covariance function of a vector variate Gaussian Process (GP) $f : \R^n \to \R^l$
be $\cov(f(\bfx), f(\bfx')) = k(\bfx, \bfx')  K^f $~\cite{bonilla2008multi},
where $k : \R^n \times \R^n
\to \R$ is scalar valued positive definite kernel function and $K^f \in \R^{l
\times l}$ is the positive-definite covariance matrix between dimensions of $f$. 
Let the training data be denoted as $\bfX := [\bfx_1^\top , \dots, \bfx_d^\top ]^\top \in
\R^{dn}$ and
corresponding output as $\bfY := [f(\bfx_1)^\top , \dots, f(\bfx_d)^\top]^\top \in
\R^{dl}$. 
Let us abbreviate $\bfk_{\bfx} := k(\bfX, \bfx)$, $\bfK_{\bfX} := K(\bfX, \bfX)$.
Then the posterior Gaussian Process $f_*(\bfx_*) := f(\bfx_*)|\bfx_*, \bfX,
\bfY$ on test point $\bfx_* $ and training data is given by
%
\begin{align}
  f_*(\bfx_*) &\sim \N\Bigl(
    % mean
  \underbrace{\left[[\bfkx \bfKX] \otimes I_{l \times l}\right] \bfY}_{\mu_f^*(\bfx_*)},
  % covar \\&
  \underbrace{[k(\bfx_*, \bfx_*) -\bfkx^\top \bfKX \bfkx]}_{k_f^*(\bfx_*, \bfx_*)} K^f
  \Bigr)
\end{align}%
% 
For proof in Section~\ref{proof:multi-variate-gp}.
\end{lemma}

If the unknown dynamics $\tdf$ and $\tdg(.)\bfu$ is learned as Vector-valued Gaussian process with
resulting means $\mutdf(\bfx)$, $\mutdgu(\bfx)$  and variances $\ktdf(\bfx, \bfx')  K^{\tdf}$, $\ktdgu(\bfx, \bfx')K^{\tdg}(\bfu, \bfu')$, respectively (computed from Lemma~\ref{thm:multi-variate-gp}).
Let the covariance between $\tdf$ and $\tdg(.)\bfu$ be denoted by 
$\cov(\tdf(\bfx), \tdg(\bfx')\bfu')$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Quadratic %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Once we know the mean, variances and covariances of each of the terms then
resulting mean and variance can be easily computed.
The mean and variance of linear combination of random vectors $Y$, with
deterministic vectors $a_i$, $b$ and $c$ can be computed by,


%
\begin{align}
  \E[X^\top Y + a^\top X+ b^\top Y + c]
  &= \E[X^\top Y] + a^\top \E[X] + b^\top \E[Y] + c \\
  \Var(X^\top Y + a^\top X+ b^\top Y + c)
  &=
    \Var(X^\top Y) + a^\top \Var(X)a + b^\top \Var(Y)b
    + 2 a^\top \cov(X, Y)b 
    \nonumber\\
  &\qquad + \cov(X^\top Y, X)^\top a  + \cov(X^\top Y, Y)^\top b
    \label{eq:linear-comb}
\end{align}
%

==> old/velocity-dependent-cbf-pendulum.tex <==
\paragraph{Velocity dependent CBF}
We assume there is a radial obstacle in the interval $(\theta_c - \Delta_{col},
\theta_c + \Delta_{col})$ that is consider the unsafe region. Thus we define the CBF
%
\begin{align}
\label{h_col}
    h(\bfx) &=\left(\cos(\Delta_{col})-\cos(\theta-\theta_c)\right)(\omega^2 + 1),
\end{align}%
%
which is non-negative when $\theta \in [0,\theta_c - \Delta_{col}] \cup [\theta_c + \Delta_{col},2\pi]$. 
\begin{remark}
  {\rm We added the multiplicative factor $\omega^2$ to $h_{col}$~\eqref{h_col}
    since in absence of it $\mathcal{L}_g h_{col}=0$, and consequently the
    condition in (...) becomes useless. }  \oprocend
\end{remark}
Thus,
\begin{align}
  \nabla_\bfx h(\bfx)&= \begin{bmatrix}
    (\omega^2 +1) \sin(\theta-\theta_c)
    \\
    2\omega\left(\cos(\Delta_{col})-\cos(\theta-\theta_c)\right)
  \end{bmatrix},
\end{align}
and 
\begin{multline}
  \mathcal{L}_f h(\bfx)= (\omega^3 + \omega) \sin(\theta-\theta_c)
  \\
  -\frac{2g\omega}{l} \sin(\theta) \left(\cos(\Delta_{col})-\cos(\theta-\theta_c)\right),
\end{multline}
\begin{multline}
    \mathcal{L}_g h(\bfx) = \\
    \begin{bmatrix}
    \frac{\omega^2 + 1}{ml}\sin(\theta - \theta_c),
    &
    \frac{2\omega}{ml} \left(\cos(\Delta_{col})-\cos(\theta-\theta_c)\right)
    \end{bmatrix}.
\end{multline}


==> tex/Inference.tex <==

\section{Matrix Variate Gaussian Process Regression of System Dynamics}
\label{learningsec:13452}
In this section we deal with the Problem~\ref{prb:learning} by developing an efficient GP framework for control-affine systems. More precisely, we use the matrix variate Gaussian (MVG) distribution~\cite{StructuredPBP} to characterize posteriors over $f$ and $g$. These posteriors will be used determine a posterior for CBC, later in Section~\ref{sec:unknowndynamics}.
\NA{I would emphasize the novelty of this section by naming and presenting it as ``Matrix Variate Gaussian Process Regression of Nonlinear Control-Affine System Dynamics''.}
%We use different methods for supervised learning Gaussian process, neural networks, Bayesian neural networks approximation (droup out), Bayesian neural networks: Deterministic Variational Inference~\cite{wu2018deterministic}.
%Let $z=(x^{\top},u^{\top})^{\top}$.
%We assume $\bar{g}u+\bar{f}=\sum_{i=1}^{\infty} \alpha_i$
%\bibliographystyle{plainnat}
%\def\localbib{\string~/wrk/group-bib/shared}
%IfFileExists{\localbib.bib}{
%\bibliography{\localbib,main_filtered}}{
%\bibliography{main_filtered}}
%The system of \eqref{eq:system_dyanmics} can written as,
%
%\begin{align}
  %\underbrace{\stdt - \barf(\state) - \barg(\state)\bfu}_{\tddotx :=} &= \tdf(\state) +  \tdg(\state) \ctrl,
  %& 
%  \bfx &= \underbrace{\begin{bmatrix}
%            f(\state)&  g(\state)
%          \end{bmatrix}}_{\dynAff(\state) :=}
 %                            \underbrace{\begin{bmatrix}1\\
                             %\ctrl\end{bmatrix}}_{\ctrlaff :=},
  %&
  %\stdt &= \dynAff(\state)\ctrlaff.
   %       \label{eq:affine-gp-cont}
%\end{align}%
% 
%We assume $\vect(\dynAff)$ to be a Gaussian process $\vect(\dynAff) \sim \GP(0,
%\kDA)$, where $\kDA$ is the vector kernel function $\kDA: \StateSp \times
%\StateSp \mapsto \R^{n(1+m) \times (1+m)n}$.
As in Coregionalization models~\cite{alvarez2012kernels} we assume the kernel of GP distribution over $\vect(F(\bfx))$, $\bfK_k(\bfx,\bfx'): \R^{n} \times
\R^{n} \mapsto \R^{n(1+m) \times (1+m)n}$, can factorized into a state dependent component $\knl_k(\state, \state')$ and a
output dimensions dependent covariance matrix $\KDA_k \in \R^{n(1+m) \times (1+m)n}$,
%
\begin{align}
\bfK_k(\bfx,\bfx') = \KDA_k \knl_k(\state, \state').
\end{align}%
% 

We note that Gaussian process $\dynAff$ is a matrix variate function and $\KDA$
can be  large matrix for high dimensional systems.
Learning the $(1+m)^2n^2$ parameters of kernel $\KDA$ requires large amount of
training data. To avoid the need of large training data, we use MVG distributions. The definition of MVG and some related results that we used in this section is detailed in
appendix~\ref{sec:MGVresutls2} for completeness. 
%\subsubsection{Matrix Variate Gaussian Process}

In line with MVG distributions,
we let 
%we define the matrix function 
%$\dynAff$ 
%\StateSp \rightarrow \R^{n \times (1+m)}$ 
%to be a MVG Process 
$F \sim \mathcal{MGP}(\bfM, \bfA, \bfB, \knl)$  with parameters
$\bfM = 0_{n \times (1+m)}$, $\bfA \in \R^{n \times n}$, 
$\bfB \in \R^{(1+m) \times (1+m)}$ and 
$\knl : \StateSp \times \StateSp \rightarrow \R^+$ is positive definite kernel,
   if 
%
\begin{align}
  \vect(\dynAff) &\sim \mathcal{GP}(\mathbf{0}, \bfK)
  &\text{where }   \bfK(\state, \state') = \KDA \knl(\state, \state') = \bfB \otimes \bfA \knl(\state, \state').
\end{align}%
% 

For training data samples, 
$\StDat_{1:k}$, let corresponding kernel
matrix be
 $\KDat := [\knl(\state_i,\state_j)]_{i=1,j=1}^{k,k}$ ,
and corresponding function values  be
$\dynAffDat(\StDat_{1:k}) := [\dynAff(\state_1), \dots, \dynAff(\state_k)] \in \R^{n \times k(1+m) }$.
An MVG Process evaluated over samples yields an MVG distribution,
%
\begin{align}
  \dynAffDat(\StDat) &\sim \mathcal{MN}(\mathbf{0}, \bfA, \KDat \otimes \bfB).
\end{align}%
% 

Let the training target data be denoted as $\StDtDat_{1:k} \in \R^{n \times k}$, and
$\CtDat_{1:k} := \diag(\ctrlaff_1, \dots, \ctrlaff_k) \in \R^{k(1+m) \times k}$.
We want to find out the function value $\dynAff(\state_*)$ at the
given test state $\state_*$.
Since $\CtDat$ is deterministic, the covariance functions of $\StDtDat_{1:k} = \dynAffDat(\StDat_{1:k}) \CtDat_{1:k}$ and $\dynAff(\state_*)$ can be written in terms of
$\KDat \otimes \bfB$, $\bfA$ and $\CtDat_{1:k}$,
%
\begin{align}
  \KDat_{\StDtDat_{1:k}}
  &:= \cov(\vect(\dynAffDat(\StDat_{1:k}) \CtDat_{1:k}),
                     \vect(\dynAffDat(\StDat_{1:k}) \CtDat_{1:k}))
                     = [ \CtDat_{1:k}^\top [ \KDat \otimes \bfB ] \CtDat_{1:k} ] \otimes \bfA
  %\\
  %&= [\knl(\bfx_i, \bfx_j)\ctrlaff_i^\top B \ctrlaff_j]_{i=1,j=1}^{k,k}  \otimes \bfA
  \\
  \kDat_{\StDtDat,*} &:= \cov(\vect(\dynAffDat(\StDat_{1:k}) \CtDat_{1:k}),
                       \vect(\dynAffDat(\state_*)))
           = [ \CtDat_{1:k}^\top [ \kDat_* \otimes \bfB ]] \otimes \bfA
  %\\
  %&= [\knl(\bfx_i, \bfx_j)\ctrlaff_i^\top B]_{i=1,j=1}^{k,k}  \otimes \bfA
  \\
  \kDat_{\dynAff_*} &:= \cov(\vect(\dynAffDat(\state_*)), \vect(\dynAffDat(\state_*)))
              = \knl(\state_*, \state_*)\bfB \otimes \bfA,
\end{align}%
% 
where $\kDat_{*} := [k(\bfx_*,\bfx_i)]_{i=1}^k$.
The train data and test data are jointly Gaussian,
%
\begin{align}
  \begin{bmatrix}
    \vect(\StDtDat_{1:k})
    \\
    \vect(\dynAff(\state_*))
  \end{bmatrix}
  \sim
  \N \left(\begin{bmatrix} \mathbf{0} \\ \mathbf{0} \end{bmatrix},
  \begin{bmatrix}
    \KDat_{\StDtDat }
    & 
    \kDat_{\StDtDat,*}
    \\
    \kDat_{\StDtDat,*}^\top
    & \kDat_{\dynAff_*}
  \end{bmatrix}
  \right).
\label{BI:GP232w}
\end{align}%
% 

Then the posterior Gaussian distribution $\vect(\dynAff^*_k(\state_*)) :=
\vect(\dynAff(\state_*)) | \state_*, \StDtDat_{1:k}, \StDat_{1:k}, \CtDat_{1:k}$ is given by,
%
\begin{align}
  \vect(\dynAff^*_k(\state_*))
  %\\
  \sim \N(
  \kDat^\top_{\StDtDat,*} \KDat_{\StDtDat}^{-1}\vect(\StDtDat_{1:k}), 
            \kDat_{\dynAff_*} - \kDat^\top_{\StDtDat,*} \KDat_{\StDtDat}^{-1} \kDat_{\StDtDat,*}).
\end{align}%
% 

The above distributions can be also written (see
Appendix~\ref{proof:matrix-variate-gp}) as an MVG distribution by
factorizing the covariance as a Kronecker product,
%
\newcommand{\mDynAffs}{\bar{\dynAff}^*_k}
\newcommand{\bfBs}{\bfB^*_k}
\begin{align}
  \dynAff^*_k(\state_*)
  %\\
  &\sim \mathcal{MN}(\mDynAffs(\bfx_*), \bfA, \bfBs(\bfx_*, \bfx_*))
  \\
  \text{where }
  \mDynAffs(\bfx_*)
  &:= \StDtDat_{1:k}
  [ \CtDat^\top [ \KDat \otimes \bfB ] \CtDat ]^{-\top}
  \CtDat^\top[ \kDat_* \otimes \bfB ]
  \\
  \bfBs(\bfx_*, \bfx_*)
  &:= \knl(\state_*, \state_*)\bfB
  - 
  [ \kDat_* \otimes \bfB ]^\top \CtDat
  \Bigl( \CtDat^\top [ \KDat \otimes \bfB ] \CtDat \Bigr)^{-1}
  \CtDat^\top [ \kDat_* \otimes \bfB ].
  \label{eq:mvg-posterior}
\end{align}
%

This can be used to compute mean and variance of $f(\bfx) + g(\bfx)\bfu$ for any deterministic $\bfu$ as,
%
\begin{align}
f(\bfx) + g(\bfx)\bfu &\sim \GP(\barf^*_k(\bfx) + \barg^*_k(\bfx)\bfu, \mathcal{K}^*_k)
\\ \text{where }
  \barf^*_k(\bfx) + \barg^*_k(\bfx)\bfu &= \mDynAffs(\bfx) \ctrlaff,
  & \mathcal{K}^*_k(\bfx, \bfx') &= \ctrlaff^\top \bfBs(\bfx, \bfx') \ctrlaff \bfA.
\label{eq:mvg-posterior-bfu-main}
\end{align}

==> tex/conditionalprobability.tex <==
\subsubsection{Proof of Theorem~\ref{safty-sampl} (The conditional safety probability)}
%\begin{proof}
Using~\eqref{eq:cbcrelations} and $\widehat{\mbox{CBC}}_k \ge \nu$ we deduce 
\begin{align}
  \mathbb{P}(\mbox{CBC}_k \ge \zeta) = \mathbb{P}(\Pi_k \le \widehat{\mbox{CBC}}_k -\zeta)
  \ge \mathbb{P}(\Pi_k \le \nu -\zeta).
\end{align}
Using Lemma~\ref{lem:NRcalculation}, $\mathbb{P}(\Pi_k \le \nu -\zeta)$ is   a cumulative distribution function (CDF) of Gussain random variable $\Pi_k$ at point $\nu -\zeta$, and the result follows.
%\end{proof}

==> tex/mean-and-variance-of-cbf-2/cbc-2-pendulum.tex <==

\paragraph{Pendulum model}
\begin{align*}
\bfx &= [\theta, \omega]
&
\bfu &= [u]
\\
f(\bfx)  &= \left[\omega, -\frac{g}{l}\sin(\theta)\right]^\top
&
g(\bfx) &= \left[0, \frac{1}{ml} \right]^\top
\\
h(\bfx) &=  \cos(\Delta_{col}) - \cos(\theta - \theta_c)
&
\grad_\bfx h(\bfx) &= \left[ \sin(\theta - \theta_c),  0 \right]^\top
\\
H_{\bfx,\bfx} h(\bfx) &= \begin{bmatrix} 
\cos(\theta - \theta_c) & 0 \\ 0 & 0\end{bmatrix}
\end{align*}

\paragraph{Computing $\CBC$}
\begin{align*}
\E[CBC ](\bfx, \bfu) &= \grad_\bfx h(\bfx)^\top \bfM(\bfx) \ctrlaff + h(\bfx)
\\
                     &=  \left[ \sin(\theta - \theta_c),  0 \right]^\top \bfM_k(\bfx) \ctrlaff + \alpha[\cos(\Delta_{col}) - \cos(\theta - \theta_c)]
\\
\Var[CBC](\bfx, \bfx'; \bfu)
&= \ctrlaff^\top \bfB_k(\bfx, \bfx')\ctrlaff 
A_{11}\sin(\theta - \theta_c)^2
\\
&= (\bfB_k(\bfx, \bfx')_{2,2}u^2 + 2\bfB_k(\bfx, \bfx')_{1,2}u + \bfB_k(\bfx, \bfx')_{1,1})
\bfA_{11}\sin(\theta - \theta_c)^2
\end{align*}

\paragraph{Computing $\CBCtwo$}

Computing $\Lie_f h(\bfx)$
\begin{align*}
 \E[\Lie_f h ](\bfx)   &= \grad h(\bfx)^\top \bfM_k(\bfx)_{:, 1}
 \\
 \Var[\Lie_f h](\bfx, \bfx') &= \bfB_k(\bfx, \bfx')_{1, 1} \grad h(\bfx)^\top \bfA \grad h(\bfx)
 \\
 &=  \bfB_k(\bfx, \bfx')_{1, 1} \bfA_{11}\sin(\theta - \theta_c)^2
 \\
 \cov(\Lie_f h, F(\bfx)\ctrlaff)
 &= B_k(\bfx, \bfx')_{1,:}^\top \ctrlaff \grad h(\bfx)^\top \bfA
 \\
 &= B_k(\bfx, \bfx')_{1,:} \ctrlaff \bfA_{1, :} \sin(\theta - \theta_c)
\end{align*}

Computing $\grad \Lie_f h(\bfx)$
\begin{align*}
 \E[\grad \Lie_f h ](\bfx)   
 &= H_{\bfx,\bfx} h(\bfx)^\top \bfM_k(\bfx)_{:, 1}
 + J^\top_\bfx \bfM_k(\bfx)_{:, 1} \grad h(\bfx)
 \\
 &= [ \cos(\theta - \theta_c) \bfM_k(\bfx)_{1,1},  0]^\top
 + J^\top_\bfx \bfM_{:,1} [\sin(\theta - \theta_c), 0]^\top
 \\
 \Var[\grad \Lie_f h](\bfx, \bfx') &= H_{\bfx,\bfx'}\bfB_k(\bfx, \bfx')_{1, 1} \grad h(\bfx)^\top \bfA \grad h(\bfx)
 \\
 &+ \grad h(\bfx')\bfA^\top H_{xx} h(\bfx) \grad_\bfx \bfB_k(\bfx, \bfx')_{1,1}
 \\
 &+ \grad_\bfx \bfB_k(\bfx, \bfx')_{1,1} \grad h(\bfx)^\top \bfA \grad h(\bfx)
 \\
 &+ \bfB_k(\bfx, \bfx')_{1,1}H_{x,x} h(\bfx) \bfA H_{x,x} h(\bfx')
 \\
 &\qquad
 \\
 &=  H_{x,x} \bfB_k(\bfx, \bfx')_{1, 1} \bfA_{11}\sin(\theta - \theta_c)^2
 \\
 &+ \grad_{\bfx} \bfB_k(\bfx, \bfx')_{1, 1} \bfA_{11} [2 \sin(\theta - \theta_c)\cos(\theta - \theta_c), 0]^\top
 \\
 &+ \bfB_k(\bfx, \bfx')_{1, 1} \bfA_{11} \begin{bmatrix}  2 \cos(\theta - \theta_c)^2 - 2 \sin(\theta - \theta_c)^2 & 0 \\ 0 & 0\end{bmatrix}
 \\
 \cov(\grad \Lie_f h, F(\bfx)\ctrlaff)
 &= B_k(\bfx, \bfx')_{1,:}^\top \ctrlaff \grad h(\bfx)^\top \bfA
 \\
 &= B_k(\bfx, \bfx')_{1,:} \ctrlaff \bfA_{1, :} \sin(\theta - \theta_c)
\end{align*}

==> tex/mean-and-variance-of-cbf-2/cbc-3-mean.tex <==
\subsection{Mean of $\CBCthree$}
\label{proof:mean-of-cbc-3}

Recall that $\grad \Lie_{\tdbff}^{(1)} h(\bfx)$ is a Gaussian Process with mean
and variance given by \eqref{eq:mean-var-grad-lie-grad-h-f},
where $\tdbff(\bfx; \bfu) = f(\bfx) + g(\bfx) \bfu$ is the control-affine
dynamics of the system which is assumed to be a Gaussian process in $\bfx$.  
We also have $\cov(\grad \Lie_{\tdbff}^{(1)} h(\bfx), \tdbff(\bfx; \bfu))$.

By definition $\Lie_{\tdbff}^{(2)} h(\bfx) := \grad[
\Lie_{\tdbff}^{(1)}h(\bfx)]^\top \tdbff(\bfx; \bfu)$. 
By using Lemma~\ref{lemma:quadratic-form}, we can compute mean and variance of 
$\Lie_{\tdbff}^{(2)} h(\bfx)$ with $\bfx = [\grad
\Lie_{\tdbff}^{(1)}h(\bfx)^\top, \tdbff(\bfx; \bfu)^\top, \Lie_{\tdbff}^{(1)}
h(\bfx)]^\top$ and $\Lambda = 0.5\begin{bmatrix} 0 & I_n & 0 \\ I_n & 0 & 0
  \\ 0 & 0 & 0\end{bmatrix}$. First note that

%
\begin{align}
  \Sigma \Lambda 
  &= 0.5\begin{bmatrix}
         \Sigma_{12} & 0 & \Sigma_{11} \\
         \Sigma_{22} & 0 & \Sigma_{21} \\
         \Sigma_{32} & 0 & \Sigma_{31}\\
    \end{bmatrix}
  &
    \Lambda \Sigma \Lambda
  & = 0.25\begin{bmatrix}
         \Sigma_{22} & 0 & \Sigma_{21} \\
         \Sigma_{12} & 0 & \Sigma_{11} \\
         0 & 0 & 0
    \end{bmatrix},
\end{align}%
% 
where $\Sigma_{11} = \Var(\grad \Lie_{\tdbff}^{(1)} h(\bfx))$, $\Sigma_{22} = \ktdbfu(\bfx, \bfx')$, $\Sigma_{12} = \Sigma_{21}^\top = \cov(\grad[ \Lie_{\tdbff}^{(1)}h(\bfx)], \tdbff(\bfx; \bfu))$, $\Sigma_{32} = \cov(\Lie_{\tdbff}^{(1)}h(\bfx), \tdbff(\bfx; \bfu))$ and $\Sigma_{31} = \cov(\Lie_{\tdbff}^{(1)}h(\bfx),\grad \Lie_{\tdbff}^{(1)}h(\bfx))$.

%
\begin{align}
    \E[\Lie_{\tdbff}^{(2)} h(\bfx)] 
    &= 
    \E[\grad \Lie_{\tdbff}^{(1)}h(\bfx)]\E[\tdbff(\bfx; \bfu)] + \tr(\cov(\grad[ \Lie_{\tdbff}^{(1)}h(\bfx)], \tdbff(\bfx; \bfu)))
    \\
    \Var[\Lie_{\tdbff}^{(2)} h(\bfx)] 
    &= 
    2\tr(\cov(\grad \Lie_{\tdbff}^{(1)}h(\bfx),\tdbff(\bfx; \bfu)))^2
    + \E[\tdbff(\bfx; \bfu)] \Var(\grad \Lie_{\tdbff}^{(1)} h(\bfx))\E[\tdbff(\bfx; \bfu)]
    \nonumber\\
    &+ \E[\grad \Lie_{\tdbff}^{(1)} h(\bfx)] \ktdbfu(\bfx, \bfx')\E[\grad \Lie_{\tdbff}^{(1)} h(\bfx)]
    \nonumber\\
    &+ 2 \E[\grad \Lie_{\tdbff}^{(1)} h(\bfx)]\cov(\grad \Lie_{\tdbff}^{(1)}h(\bfx),\tdbff(\bfx; \bfu))\E[\tdbff(\bfx; \bfu)]
    \\
    \cov(\Lie_{\tdbff}^{(2)} h(\bfx), \tdbff(\bfx; \bfu)) 
    &= \cov(\grad \Lie_{\tdbff}^{(1)}h(\bfx),\tdbff(\bfx; \bfu))\E[\tdbff(\bfx; \bfu)] + \knl(\bfx, \bfx') \E[\grad \Lie_{\tdbff}^{(1)} h(\bfx)]
    \\
    \cov(\Lie_{\tdbff}^{(2)} h(\bfx), \Lie_{\tdbff}^{(1)}(\bfx))
    &= \cov(\Lie_{\tdbff}^{(1)}h(\bfx),\grad \Lie_{\tdbff}^{(1)}h(\bfx))\E[\tdbff(\bfx; \bfu)] 
    + \cov(\Lie_{\tdbff}^{(1)}h(\bfx), \tdbff(\bfx; \bfu)) \E[\grad \Lie_{\tdbff}^{(1)} h(\bfx)]
\end{align}
%

Note that $\Lie_{\tdbff}^{(2)} h(\bfx)$ is no longer a Gaussian process.
However, both Lemma~\ref{lemma:differentiating-gp} and the expectation part of Lemma~\ref{lemma:quadratic-form}   
are valid for any random process with finite mean and variance.
For this reason the expectation recursive formula is true for arbitrary relative degree $r$,

%
\begin{align}
    \E[\Lie_{\tdbff}^{(r+1)} h(\bfx)] 
    &= 
    \E[\grad \Lie_{\tdbff}^{(r)}h(\bfx)]\E[\tdbff(\bfx; \bfu)] + \tr(\cov(\grad[ \Lie_{\tdbff}^{(r)}h(\bfx)], \tdbff(\bfx; \bfu)))
\end{align}
%
However for $r >= 3$, it is harder to compute $\cov(\grad[ \Lie_{\tdbff}^{(r)}h(\bfx)], \tdbff(\bfx; \bfu))$.
But for $r=3$, we know  $\cov(\grad \Lie_{\tdbff}^{(2)} h(\bfx), \tdbff(\bfx; \bfu)) = \grad \cov(\Lie_{\tdbff}^{(2)} h(\bfx), \tdbff(\bfx; \bfu))$ from Lemma~\ref{lemma:differentiating-gp} which is valid for any random process, not just Gaussian process,
%
\begin{align}
    \E[\Lie_{\tdbff}^{(3)} h(\bfx)] 
    &= 
    \E[\grad \Lie_{\tdbff}^{(2)}h(\bfx)]\E[\tdbff(\bfx; \bfu)] + \tr(\grad\cov( \Lie_{\tdbff}^{(2)}h(\bfx), \tdbff(\bfx; \bfu)))
\end{align}
%

Now $\CBCthree(\bfx; \bfu)$ can be written in terms $\Lie_{\tdbff}^{(3)}
h(\bfx)$,
%
\begin{align}
  \CBCthree(\bfx; \bfu) = \Lie_{\tdbff}^{(3)} h(\bfx)
  + K_\alpha \begin{bmatrix}
    h(\bfx) \\ \Lie_{\tdbff}^{(1)} h(\bfx) \\ \Lie_{\tdbff}^{(2)} h(\bfx) \ge 0
    \end{bmatrix}.
\end{align}%
% 
The expectation of $\CBCthree$ is simply the linear combination of the
expectations,
%
\begin{align}
  \E[\CBCthree(\bfx; \bfu)] = \E[\Lie_{\tdbff}^{(3)} h(\bfx)]
  + K_{\alpha,1} h(\bfx)
  + K_{\alpha,2} \E[\Lie_{\tdbff}^{(1)} h(\bfx)]
  + K_{\alpha,3} \E[\Lie_{\tdbff}^{(2)} h(\bfx)] \ge 0
\end{align}%
% 




==> tex/mean-and-variance-of-cbf-2/cbf-2-affine-quadratic.tex <==
\subsubsection{Mean is affine and Variance is quadratic}
\label{proof:mean-affine-var-quadratic}
Next we want to see if the mean and variance are quadratic or higher in $\bfu$.
Expanding each term in $\mCBCtwo$.

%
\begin{align}
  \bar{\bfz}(\bfx; \bfu)\Lambda \bar{\bfz}(\bfx; \bfu)
  &= \grad \tdLie_f h(\bfx)^\top \mDynAffs(\bfx)\ctrlaff
  \\
  \tr(\Lambda \Sigma_\bfz(\bfx, \bfx; \bfu))
  &= \tr(\cov(\grad \tdLie_fh(\bfx), \hDynAff(\bfx)\ctrlaff))
  \\
  &= \tr(\grad_\bfx \ktdfbfu(\bfx,\bfx')\ctrlaff\grad h(\bfx)^\top 
    + \ktdfbfu(\bfx,\bfx')\ctrlaff H_{xx} h(\bfx)^\top)
  \\
  \bfd(\bfx; \bfu)^\top\bar{\bfz}(\bfx; \bfu)
  &= 
    \grad \bLie_{f} h(\bfx)^\top \mDynAffs(\bfx)\ctrlaff
    + \overline{\grad \tdLie_f h(\bfx)}^\top [ \barf(\bfx) + \barg(\bfx)\bfu ] 
    + K_{\alpha,2}\overline{\tdLie_f h(\bfx)}
\end{align}%
% 
Hence, the expectation $\mCBCtwo$ is actually control-affine,
%
\begin{multline}
\mCBCtwo = \grad \tdLie_f h(\bfx)^\top \mDynAffs(\bfx)\ctrlaff
\\
    + \grad_\bfx \ktdfbfu(\bfx,\bfx')\ctrlaff\grad h(\bfx)^\top 
    + \ktdfbfu(\bfx,\bfx')\ctrlaff H_{xx} h(\bfx)^\top
    \\
    + \grad \bLie_{f} h(\bfx)^\top \mDynAffs(\bfx)\ctrlaff
    + \overline{\grad \tdLie_f h(\bfx)}^\top [ \barf(\bfx) + \barg(\bfx)\bfu ] 
    + K_{\alpha,2}\overline{\tdLie_f h(\bfx)}
    \\
+ \grad \bLie_{f} h(\bfx)^\top[ \barf(\bfx) + \barg(\bfx)\bfu ]
+ K_{\alpha,1} h(\bfx) + K_{\alpha,2} \bLie_{f} h(\bfx)
\end{multline}%
% 

Next we expand each term in $\VCBCtwo$ to see if it is quadratic in control $\bfu$.
%
\begin{align}
  2\tr(\Lambda \Sigma_\bfz(\bfx, \bfx; \bfu))^2
  &= \tr(\cov(\grad \tdLie_fh(\bfx), \hDynAff(\bfx)\ctrlaff))
\end{align}
\begin{align}
  \Lambda \Sigma_\bfz(\bfx, \bfx; \bfu) \Lambda
  &=
    \begin{bmatrix}
      0.5\cov(\grad \tdLie_f h(\bfx), \hDynAff(\bfx)\ctrlaff)
      &  0.5\ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff
      & 0.5 \cov(\tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
      \\
      0.5K_{\grad \tdLie_f h}(\bfx, \bfx')
      & 0.5\cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
      & 0.5\cov(\grad \tdLie_f h(\bfx), \tdLie_f h(\bfx))
    \\
    0 & 0 & 0
  \end{bmatrix} \Lambda
  \nonumber\\
  &=
    \begin{bmatrix}
      0.25\ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff
      & 0.25\cov(\grad \tdLie_f h(\bfx), \hDynAff(\bfx)\ctrlaff)
      & 0
      \\
      0.25\cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
      & 0.25K_{\grad \tdLie_f h}(\bfx, \bfx')
      & 0
    \\
    0 & 0 & 0
  \end{bmatrix}
  \\
  4\bar{\bfz}(\bfx; \bfu)^\top \Lambda
  \Sigma_\bfz&(\bfx, \bfx; \bfu) \Lambda \bar{\bfz}(\bfx; \bfu)
               = 
\grad \tdLie_f h(\bfx)^\top \ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff \grad \tdLie_f h(\bfx)
  \nonumber\\
  &
    + 2\grad \tdLie_f h(\bfx)^\top \cov(\grad \tdLie_f h(\bfx), \hDynAff(\bfx)\ctrlaff)  \hDynAff(\bfx)\ctrlaff
  \nonumber\\
  &
    +  \ctrlaff^\top\hDynAff(\bfx)^\top K_{\grad \tdLie_f h}(\bfx, \bfx') \hDynAff(\bfx)\ctrlaff
\end{align}
\begin{align}
  \bfd(\bfx; \bfu)^\top
  \Sigma_\bfz&(\bfx, \bfx; \bfu) \bfd(\bfx; \bfu)
               =
               (\barf(\bfx) + \barg(\bfx)\bfu)^\top K_{\grad \tdLie_f h}(\bfx, \bfx')(\barf(\bfx) + \barg(\bfx)\bfu)
  \nonumber\\
             &+ \grad \bLie_f h(\bfx)^\top\ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff \grad \bLie_f h(\bfx)
  \nonumber\\
  &+ K_{\alpha,2} \knl_{\tdLie_f h}(\bfx, \bfx') K_{\alpha,2}
  \nonumber\\
  &+ 2(\barf(\bfx) + \barg(\bfx)\bfu)^\top \cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))^\top \grad \bLie_f h(\bfx)
  \nonumber\\
  &+ 2(\barf(\bfx) + \barg(\bfx)\bfu)^\top \cov(\grad \tdLie_f h(\bfx), \tdLie_f h(\bfx))  K_{\alpha,2}
  \nonumber\\
  &+ 2\grad \bLie_f h(\bfx)^\top\ctrlaff^\top\cov(\tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))^\top    K_{\alpha,2}
\end{align}%
% 
%
\begin{align}
  4 \bfd(\bfx; \bfu)^\top
  & \Sigma_\bfz(\bfx, \bfx; \bfu) \Lambda \bar{\bfz}(\bfx; \bfu)
  = 2 \bfd(\bfx; \bfu)
  \begin{bmatrix}
    \cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
    & K_{\grad \tdLie_f h}(\bfx, \bfx')
    & 0 \\
    \ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff
    & \cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))^\top
    &  0 \\
    \cov(\grad \tdLie_f h(\bfx), \tdLie_f h(\bfx))^\top
    & \cov(\tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
    &  0
  \end{bmatrix}
      \bar{\bfz}(\bfx; \bfu)
  \nonumber\\
  &= (\barf(\bfx) + \barg(\bfx)\bfu)^\top
    \cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
    \grad \tdLie_f h(\bfx)
    \nonumber\\
  &+ (\barf(\bfx) + \barg(\bfx)\bfu)^\top
  K_{\grad \tdLie_f h}(\bfx, \bfx')
  \hDynAff(\bfx)\ctrlaff
    \nonumber\\
  &+ \grad \bLie_f h(\bfx)^\top
    \ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff
    \grad \tdLie_f h(\bfx)^\top
    \nonumber\\
    &+ \grad \bLie_f h(\bfx)^\top
      \cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))^\top
      \hDynAff(\bfx)\ctrlaff
    \nonumber\\
    &+ K_{\alpha,2}
    \cov(\grad \tdLie_f h(\bfx), \tdLie_f h(\bfx))^\top
    \grad \tdLie_f h(\bfx)
    \nonumber\\
  &+ K_{\alpha,2}\cov(\tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
      \hDynAff(\bfx)\ctrlaff
\end{align}%
% 
Since all the terms at most quadratic in $\bfu$, this means that $\VCBCtwo$ is
quadratic in $\bfu$.

==> tex/mean-and-variance-of-cbf-2/covar-of-jac-of-gp.tex <==
\begin{lemma}[Covariance matrix of Jacobian of Gaussian Process]
  \label{lemma:covar-of-jac-of-gp}
Under assumptions of Lemma~\ref{thm:mean-of-jac-of-gp}, the covariance matrix of
the vectorized $\vect(J_{\bfx_*} f_*(\bfx_*)) \in \R^{ln}$ is given by,
% 
  \begin{align}
    \Cov(\bfj_*, \bfj'_*) &=
    \left[ H_{xx} k(\bfx_*, \bfx'_*)
    - J_{\bfx_*}^\top \bfkx\bfKX J_{\bfx_*}\bfkxp \right] \otimes K^f
  \end{align}%
  % 
  For scalar-valued GP, $K^f = 1$,
% 
  \begin{align}
    \Cov(\bfj_*, \bfj'_*) &= H_{xx} k(\bfx_*, \bfx'_*) - J_{\bfx_*}^\top \bfkx\bfKX J_{\bfx_*}\bfkxp
  \end{align}%
  % 
  For proof see Section~\ref{proof:covar-of-jac-of-gp}.
\end{lemma}%
% 

\subsubsection{Covariance matrix of Jacobian of GP (Lemma~\ref{lemma:covar-of-jac-of-gp})}
\label{proof:covar-of-jac-of-gp}
\newcommand{\bbfj}{\bar{\bfj}}

Before computing variance, without loss of generality, we consider $J_\bfx f_*(\bfx_*)$
with zero mean.
We write the covariance matrix for $\bfj_* := \vect(J_{\bfx_*} f_*(\bfx_*))$,
% E[fᵢ/x₂, f₃/x₄]
\newcommand{\Epf}[4]{\E\left[\frac{\p f_{#1,*}}{\p x_{#2,*}} \frac{\p f_{#3,*}}{\p x_{#4,*}}\right]}
% E[f/x₁, f/x₂]
\newcommand{\Epbf}[2]{\E\left[\frac{\p \bff_{*}}{\p x_{#1,*}} \frac{\p \bff^\top_{*}}{\p x_{#2,*}}\right]}
%
\begin{align}
  \Cov(\bfj_*, \bfj_*) &:= \E[\bfj_*\bfj_*^\top]
  \\
  \E[\bfj_*\bfj_*^\top] &= \begin{bmatrix}
    \Epbf{1}{1} & \dots & \Epbf{1}{n}
    \\ \vdots & & \vdots \\
    \Epbf{n}{1} & \dots & \Epbf{n}{n}
  \end{bmatrix}
  \\
  \text{where } \Epbf{i}{j} &= \begin{bmatrix}
    \Epf{1}{i}{1}{j} & \dots & \Epf{1}{i}{l}{j}
    \\ \vdots & & \vdots \\
    \Epf{l}{i}{1}{j} & \dots & \Epf{l}{i}{l}{j}
  \end{bmatrix},
\end{align}
%
and we have abbreviated $\bff_* = f_*(\bfx_*)$.

% E[fᵢ/x, fⱼ/x]
\newcommand{\Epfbx}[2]{\E\left[\frac{\p f_{#1,*}}{\p \bfx_{*}} \frac{\p f_{#2,*}}{\p \bfx'_{*}}^\top\right]}
Let us compute the value of $\Epfbx{i}{j}$,

%
\newcommand{\dbfx}{\delta\bfx}
\begin{align}
  \Epfbx{i}{j} &= \lim_{\dbfx,\dbfx' \to 0}\E\left[
  \frac{f_{i,*}(\bfx_* + \dbfx) - f_{i,*}(\bfx_*)}{\dbfx}
  \frac{f_{j,*}(\bfx'_* + \dbfx') - f_{j,*}(\bfx'_*)}{\dbfx'}
  \right]
  \\
               &= \lim_{\dbfx,\dbfx' \to 0}
                 \E\left[\frac{f_{i,*}(\bfx_* + \dbfx)f_{j,*}(\bfx'_* + \dbfx')}{\dbfx \dbfx'}\right]
                 + \E\left[\frac{f_{i,*}(\bfx_*)f_{j,*}(\bfx'_*)}{\dbfx \dbfx'}\right]
  \nonumber\\
               &- \E\left[\frac{f_{i,*}(\bfx_* + \dbfx)f_{j,*}(\bfx'_*)}{\dbfx \dbfx'}\right]
                 - \E\left[\frac{f_{i,*}(\bfx_* )f_{j,*}(\bfx'_* + \dbfx'_*)}{\dbfx \dbfx'}\right]
\end{align}
Note that from Lemma~\ref{thm:multi-variate-gp}, $\E[f_i(\bfx)f_j(\bfx')] =
(k(\bfx, \bfx') - k(\bfx, \bfX)K(\bfX, \bfX)^{-1}k(\bfX, \bfx')) K^f_{i,j}$.
\newcommand{\bfkxd}{\bfk_{\bfx_* + \dbfx}}
\newcommand{\bfkxpd}{\bfk_{\bfx'_* + \dbfx'}}
\begin{align}
  \Epfbx{i}{j}
               &= \lim_{\dbfx,\dbfx' \to 0}
                 \frac{k(\bfx_* + \dbfx, \bfx'_* + \dbfx')
                 - \bfkxd^\top\bfKX\bfkxpd}{\dbfx \dbfx'}K^f_{i,j}
                 \nonumber \\
               & \quad + \frac{k(\bfx_*, \bfx'_*) - \bfkx^\top\bfKX\bfkxp}{\dbfx \dbfx'}K^f_{i,j}
                 - \frac{k(\bfx_* + \dbfx,\bfx'_*)-\bfkxd^\top \bfKX\bfkxp}{\dbfx \dbfx'}K^f_{i,j}
                 \nonumber \\
               & \quad - \frac{k(\bfx_*, \bfx'_* + \dbfx'_*)-\bfkx^\top \bfKX\bfkxpd}{\dbfx \dbfx'}K^f_{i,j}
    %
  \\
  % Arrange terms to look like derivatives
               &= K^f_{i,j}\lim_{\dbfx,\dbfx' \to 0}
                 \frac{1}{\dbfx}\frac{k(\bfx_* + \dbfx, \bfx'_* + \dbfx') - k(\bfx_* + \dbfx,\bfx'_*)}{\dbfx'}
                 \nonumber\\
               & \quad - \frac{1}{\dbfx}\frac{k(\bfx_*, \bfx'_* + \dbfx'_*) - k(\bfx_*, \bfx'_*)}{\dbfx'}
                 - \left(\frac{\bfkxd^\top\bfKX }{\dbfx}\frac{\bfkxpd -  \bfkxp}{\dbfx'} \right)
                 \nonumber \\
                 &\quad+  \left(\frac{\bfkx^\top\bfKX}{\dbfx}\frac{\bfkxpd - \bfkxp}{\dbfx'} \right)
                 % 
  \\
  % Replace with derivatives
               &= K^f_{i,j}\lim_{\dbfx \to 0}
                 \frac{1}{\dbfx}\frac{\p k(\bfx_* + \dbfx, \bfx'_*)}{\p \bfx}
                 - \frac{1}{\dbfx}\frac{\p k(\bfx_*, \bfx'_*)}{\p \bfx}
                 \nonumber \\
               & \quad- \left(\frac{\bfkxd - \bfkx}{\dbfx} \right)^\top \bfKX \frac{\p \bfkxp}{\p \bfx}
  \\
  % Final result
               &= \left( \frac{\p^2 k(\bfx_*, \bfx'_*)}{\p \bfx_*^2}
                 - \frac{\p \bfkx^\top}{\p \bfx}\bfKX \frac{\p \bfkxp}{\p \bfx} \right)K^f_{i,j}. 
\end{align}%
% 
The result is a matrix whose $p,q$ is,
%
\begin{align}
  \Epf{i}{p}{j}{q} = \left[\Epfbx{i}{j}\right]_{p,q} =
  \left[ \frac{\p^2 k(\bfx_*, \bfx'_*)}{\p \bfx_*^2}
                 - \frac{\p \bfkx^\top}{\p \bfx}\bfKX \frac{\p \bfkxp}{\p \bfx} \right]_{p,q}K^f_{i,j}
\end{align}%
% 
Now, we can construction $\Epbf{p}{q}$,
%
\begin{align}
\Epbf{p}{q} &= 
  \left[ \frac{\p^2 k(\bfx_*, \bfx'_*)}{\p \bfx_*^2}
                 - \frac{\p \bfkx^\top}{\p \bfx}\bfKX \frac{\p \bfkxp}{\p \bfx} \right]_{p,q}K^f
\end{align}%
% 
Hence, the full covariance matrix becomes,
%
\begin{align}
\Cov(\bfj_*, \bfj_*) &= 
  \left[ \frac{\p^2 k(\bfx_*, \bfx'_*)}{\p \bfx_*^2}
                 - \frac{\p \bfkx^\top}{\p \bfx}\bfKX \frac{\p \bfkxp}{\p \bfx} \right] \otimes K^f
  \\
  &= \left[ H_{xx} k(\bfx_*, \bfx'_*)
    - J_{\bfx_*}^\top \bfkx\bfKX J_{\bfx_*}\bfkxp \right] \otimes K^f
\end{align}%
% 

\hfill $\blacksquare $

==> tex/mean-and-variance-of-cbf-2/mean-of-jac-of-gp.tex <==
%
\begin{lemma}[Mean of Jacobian of Gaussian Process]
  \label{thm:mean-of-jac-of-gp}
Under assumptions of Lemma~\ref{thm:multi-variate-gp}, the Jacobian of
posterior GP, $J_{\bfx_*} f_*(\bfx) \in \R^{l \times n}$, is also Gaussian.
The mean of the vectorized $\bfj_* := \vect(J_{\bfx_*} f_*(\bfx_*)) \in \R^{ln}$ is given by,
% 
  \begin{align}
    \bar{\bfj}_* := \E[\vect(J_{\bfx_*} f_*(\bfx_*))] &= \left[[J_{\bfx_*}^\top \bfkx \bfKX] \otimes I_{l \times l}\right] \bfY.
  \end{align}%
  % 
  For scalar-valued GP put $l=1$, 
% 
  \begin{align}
    \bar{\bfj}_* := \E[\grad_\bfx f_*(\bfx_*)] &= J_{\bfx_*}^\top \bfkx \bfKX \bfY.
  \end{align}%
  % 
  For proof see Section~\ref{proof:mean-of-jac-of-gp}.
\end{lemma}%
% 

\subsubsection{Mean of Jacobian of Gaussian process(Lemma~\ref{thm:mean-of-jac-of-gp})}
\label{proof:mean-of-jac-of-gp}
Since jacobian is a linear operator, we can compute the mean by swapping
expectation and jacobian,
%
\begin{align}
  \E[\vect(J_{\bfx_*} f_*(\bfx_*))] &= \vect(J_{\bfx_*} \E[f_*(\bfx)]) =
                          \vect\left( J_{\bfx_*} \left\{ \left[[k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY \right\} \right)
\end{align}


\begin{align}
  \E[\vect(J_{\bfx_*} f_*(\bfx_*))] =
  \vect\Bigl( J_{\bfx_*}& \left\{ \left[[k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY \right\} \Bigr)
  \\
                        &= \begin{bmatrix}
                          \frac{\p }{\p x_{1,*}} \left[[k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY
                          \\ \vdots \\
                          \frac{\p }{\p x_{n,*}} \left[[k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY
                        \end{bmatrix}
  \\
                        &= \begin{bmatrix}
                          \left[[\frac{\p }{\p x_{1,*}} k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY
                          \\ \vdots \\
                          \left[[\frac{\p }{\p x_{n,*}} k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY
                        \end{bmatrix}
  \\
                        &= \begin{bmatrix}
                          [\frac{\p }{\p x_{1,*}} k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}
                          \\ \vdots \\
                          [\frac{\p }{\p x_{n,*}} k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}
                          \end{bmatrix} \bfY
  \label{eq:mean-jac-pre-vcat}
\end{align}

Consider the Kronecker product of vertical concatenation of matrices,
%
\begin{align}
  \begin{bmatrix} A \otimes B \\ C \otimes B\end{bmatrix}
  = \begin{bmatrix}
    A_{11}B & \dots & A_{1n} B
    \\ \vdots && \vdots \\
    A_{n1}B & \dots & A_{nn} B \\
    C_{11}B & \dots & C_{1n} B
    \\ \vdots && \vdots \\
    C_{n1}B & \dots & C_{nn} B \\
  \end{bmatrix}
  = \begin{bmatrix} A \\ C \end{bmatrix} \otimes B
  \label{eq:prop-kronecker-vcat}
\end{align}%
% 

Apply property \eqref{eq:prop-kronecker-vcat} to \eqref{eq:mean-jac-pre-vcat},
%
\begin{align}
  \E[\vect(J_{\bfx_*} f_*(\bfx_*))] &= \begin{bmatrix}
    \left[ \begin{bmatrix}
      \frac{\p }{\p x_{1,*}} k(\bfx_*, \bfX)
      \\ \vdots \\
      \frac{\p }{\p x_{n,*}} k(\bfx_*, \bfX)
    \end{bmatrix}
    K(\bfX, \bfX)^{-1} \right] \otimes I_{l \times l}
    \end{bmatrix}\bfY
\end{align}%
% 

\begin{align}
  \E[\vect(J_{\bfx_*} f_*(\bfx_*))]
  &= \left[[J_{\bfx_*}^\top k(\bfx_*, \bfX) K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY
  \\
  &= \left[[J_{\bfx_*}^\top \bfkx \bfKX] \otimes I_{l \times l}\right] \bfY.
\end{align}
\hfill $\blacksquare $

==> tex/mean-and-variance-of-cbf-2/multi-variate-gp.tex <==
\subsubsection{Multi-variate Gaussian Process (Eq~\eqref{eq:mvg-posterior})}
\label{proof:multi-variate-gp}

Consider $f(\bfx_i) = \vect{\dynAff(\bfx_i)}$ and $K^f = \bfB \otimes \bfA \in
\R^l$, where $l = mn$.
Then $f(\bfx, \bfx') \sim \GP(0, k(\bfx, \bfx')K^f)$.

\newcommand{\bfkx}{\bfk_{\bfx_*}}
\newcommand{\bfKX}{\bfK^{-1}_\bfX}
\newcommand{\bfkxp}{\bfk_{\bfx'_*}}

The joint distribution between test data and train data is Gaussian,
%
\begin{align}
  \begin{bmatrix}
    f(\bfx_1)
    \\ \vdots \\
    f(\bfx_d)
    \\
    f(\bfx_*)
  \end{bmatrix}
  &\sim
  \N\left(
  % mean
  \begin{bmatrix}
    \mathbf{0}_{l}
    \\ \vdots \\
    \mathbf{0}_{l}
    \\
    \mathbf{0}_{l}
  \end{bmatrix},
  % covar
  \begin{bmatrix}
    k(\bfx_1, \bfx_1)K^f & \dots & k(\bfx_1, \bfx_d)K^f & k(\bfx_1, \bfx_*) K^f
    \\ \vdots & & \vdots & \vdots \\
    k(\bfx_d, \bfx_1)K^f & \dots & k(\bfx_d, \bfx_d)K^f & k(\bfx_d, \bfx_*) K^f
    \\
    k(\bfx_*, \bfx_1)K^f & \dots & k(\bfx_*, \bfx_d)K^f & k(\bfx_*, \bfx_*) K^f
  \end{bmatrix}
                                                          \right)
  \\
  \begin{bmatrix}
    \bfY
    \\
    f(\bfx_*)
  \end{bmatrix}
  &\sim
  \N\left(
  % mean
  \begin{bmatrix}
    \mathbf{0}_{dl}
    \\
    \mathbf{0}_{l}
  \end{bmatrix},
  % covar
  \begin{bmatrix}
    K(\bfX, \bfX) \otimes K^f & k(\bfX, \bfx_*) \otimes K^f
    \\
    k(\bfx_*, \bfX) \otimes K^f & k(\bfx_*, \bfx_*) \otimes K^f
  \end{bmatrix}
                                                          \right),
\end{align}%
% 
where $k(\bfx_*, \bfX) := [k(\bfx_*, \bfx_1), \dots, k(\bfx_*, \bfx_d)]^\top =:
k(\bfX, \bfx_*)^\top$, and $K(\bfX, \bfX) := [k(\bfx_i, \bfx_j)]_{i=1,j=1}^{n,n}$.

The posterior of GP on a test point $\bfx_*$ is given by,
%
\begin{align}
  f_*(\bfx_*) := f(\bfx_*) | \bfX, \bfY &\sim \N\Bigl(
    % mean
  (k(\bfx_*, \bfX) \otimes K^f) (K(\bfX, \bfX)  \otimes K^f)^{-1} \bfY,
  % covar
  \\&
  (k(\bfx_*, \bfx_*) \otimes K^f) -
  (k(\bfx_*, \bfX) \otimes K^f) (K(\bfX, \bfX)  \otimes K^f)^{-1} (k(\bfX, \bfx_*) \otimes K^f)
  \Bigr).
\end{align}%
% 

By using properties of Kronecker product
$(A \otimes B)(C \otimes D) = AC \otimes BD$,
$(A \otimes B)^{-1} = A^{-1} \otimes B^{-1}$,
$(A \otimes C + B \otimes C) = (A + B) \otimes C$, we get
%
%
\begin{align}
  f_*(\bfx_*)
  & \sim \N\Bigl(
  % mean
  \left[[k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l}\right] \bfY,
  % covar \\&
  [k(\bfx_*, \bfx_*) -k(\bfx_*, \bfX) K(\bfX, \bfX)^{-1} k(\bfX, \bfx_*)] K^f
  \Bigr)
  \\
  &=
    \N\Bigl(
    % mean
  \left[[\bfkx \bfKX] \otimes I_{l}\right] \bfY,
  % covar \\&
  [k(\bfx_*, \bfx_*) -\bfkx^\top \bfKX \bfkx] K^f
  \Bigr),
\end{align}%
% 
where $I_{l} \in \R^{l}$ is identity matrix.

Substitute $K^f = \bfB \otimes \bfA$ and $I_l = I_n \otimes I_m$.
\hfill  $ \blacksquare $

==> tex/mean-and-variance-of-cbf-2/positive-definiteness.tex <==
\subsubsection{Is the deterministic condition positive-definite?}
For a relative degree 2 system, we can write $\CBCtwo$ as 


==> tex/mean-and-variance-of-cbf-2/sanity-check.tex <==
\subsubsection{Sanity check for matrix calculus \eqref{eq:grad-of-lie-h}}
\label{proof:grad-of-lie-h}


%
\begin{align}
  \grad_\bfx \Lie_fh(\bfx)^\top &= \grad_\bfx [ \grad_\bfx h(\bfx)^\top f(\bfx) ]
                             %
  =\begin{bmatrix} \frac{\p \Lie_fh(\bfx)}{\p x_1}
    &\dots & \frac{\p \Lie_fh(\bfx)}{\p x_n}
    \end{bmatrix}
      %
\end{align}%
% 

Computing derivatives element wise,
%
\begin{align}
  \Lie_fh(\bfx) &= \grad_\bfx h(\bfx)^\top f(\bfx) = f_1(\bfx) \frac{\p h}{\p x_1}
  + \dots + f_n(\bfx) \frac{\p h}{\p x_n}
  \\
  \grad_\bfx \Lie_fh(\bfx) &= \begin{bmatrix}
    \frac{\p f_1}{\p x_1} \frac{\p h}{\p x_1}
    + f_1(\bfx) \frac{\p^2 h}{\p x_1 \p x_1}
    + \dots
    + \frac{\p f_n}{\p x_1} \frac{\p h}{\p x_n}
    + f_n(\bfx) \frac{\p^2 h}{\p x_1 \p x_n}
    \\
    \vdots
    \\
    \frac{\p f_1}{\p x_n} \frac{\p h}{\p x_1}
    + f_1(\bfx) \frac{\p^2 h}{\p x_n \p x_1}
    \dots
    + \frac{\p f_n}{\p x_n} \frac{\p h}{\p x_n}
    + f_n(\bfx) \frac{\p^2 h}{\p x_n \p x_n}
    \end{bmatrix}
  \label{eq:sanity-elementwise}
\end{align}%
% 

Computing derivatives by matrix calculus,
%
\begin{align}
  \grad_\bfx \Lie_fh(\bfx) &= \grad_\bfx [\grad_\bfx h(\bfx)^\top f(\bfx)]
                       = H_{xx}h(\bfx) f(\bfx)  + J_x^\top f(\bfx)\grad_\bfx h(\bfx)
  \\
               &= \begin{bmatrix}
                 f_1(\bfx)\frac{\p^2 h}{\p x_1 \p x_1}
                 + \dots + f_n(\bfx)\frac{\p^2 h}{\p x_1 \p x_n}
                 \\ \vdots \\
                 f_1(\bfx)\frac{\p^2 h}{\p x_n \p x_1}
                 + \dots + f_n(\bfx)\frac{\p^2 h}{\p x_n \p x_n}
               \end{bmatrix}
                   +
                   \begin{bmatrix}
                     \frac{\p h}{\p x_1}\frac{\p f_1}{\p x_1}
                     + \dots + \frac{\p h}{\p x_n}\frac{\p f_n}{\p x_1}
                     \\ \vdots \\
                     \frac{\p h}{\p x_1}\frac{\p f_1}{\p x_n}
                     + \dots + \frac{\p h}{\p x_n}\frac{\p f_n}{\p x_n}
                   \end{bmatrix}
  \\
               &= \begin{bmatrix}
                 f_1(\bfx)\frac{\p^2 h}{\p x_1 \p x_1}
                 + f_n(\bfx)\frac{\p^2 h}{\p x_1 \p x_n}
                 + \dots + \frac{\p h}{\p x_1}\frac{\p f_1}{\p x_1}
                 + \frac{\p h}{\p x_n}\frac{\p f_n}{\p x_1}
                 \\ \vdots \\
                 f_1(\bfx)\frac{\p^2 h}{\p x_n \p x_1}
                 + f_n(\bfx)\frac{\p^2 h}{\p x_n \p x_n}
                 + \dots + \frac{\p h}{\p x_1}\frac{\p f_1}{\p x_n}
                 + \frac{\p h}{\p x_n}\frac{\p f_n}{\p x_n}
               \end{bmatrix}
  \label{eq:sanity-matrix-calculus}
\end{align}%
% 
Terms \eqref{eq:sanity-matrix-calculus} and \eqref{eq:sanity-elementwise} are
the same.
\hfill $\blacksquare $

==> tex/mean-and-variance-of-cbf-r-diagram.tex <==
\usetikzlibrary{positioning}
\begin{tikzpicture}[]
\providecommand{\bfx}{\mathbf{x}}
\providecommand{\Lie}{\mathcal{L}}
\providecommand{\grad}{\nabla}
\node [] (h) {$h(\bfx)$};

\node [right=of h] (gh) {$\grad h(\bfx)$};

\path[->] (h)  edge [above] node {$\nabla$} (gh);

\node [right=of gh] (L1) {$\Lie_f^{(1)} h(\bfx)$};

\node [below= of L1] (f1) {$f(\bfx)$};

\path[->] (f1)  edge (L1);

\path[->] (gh)  edge (L1);

\node [right=of L1] (gL1) {$\grad \Lie_f^{(1)} h(\bfx)$};

\path[->] (L1)  edge [above] node {$\nabla$} (gL1);

\node [right=of gL1] (L2) {$\Lie_f^{(2)} h(\bfx)$};

\node [below= of L2] (f2) {$f(\bfx)$};

\path[->] (f2)  edge (L2);

\path[->] (gL1)  edge (L2);

\node [right=of L2] (gL2) {};
\draw[dotted] (L2) -- (gL2) ;

\end{tikzpicture}

==> tex/mean-and-variance-of-cbf-r.tex <==
Let the kernel of the dynamics $f(\bfx)$ be an exponential kernel. It can be
shown that the double derivative of the exponential kernel is the kernel itself
with a scale factor

\begin{lemma}[Double derivative of exponential kernel]
  If $\knl(\bfx_1, \bfx_2) = \exp(-0.5(\bfx_1 - \bfx_2)\Sigma^{-1}(\bfx_1 -
  \bfx_2))$, then
  \begin{align}
    \frac{\partial^2 \knl(\bfx_1, \bfx_2)}
    {\partial \bfx_1 \partial \bfx_2} \Big|_{\bfx_1 = \bfx_2}
    &= \Sigma^{-1} \knl(\bfx_1, \bfx_2)
  \end{align}%
\end{lemma}%
%

Let the Control Barrier Function $h(\bfx)$ be of degree $r$, i.e.
$\Lie_g^{(r-1)} h(\bfx) = 0$, then the $(r-1)$th Lie derivative of $f(\bfx)$ is
given by the following recursive formula

%
\begin{align}
  \Lie_f^{(1)} h(\bfx) &= \grad_\bfx [h(\bfx)]^\top f(\bfx)
  \\
  \Lie_f^{(i+1)} h(\bfx) &= \grad_\bfx [\Lie_f^{(i)} h(\bfx)]^\top f(\bfx) \qquad \forall i \in \{ 1, \dots, r-1 \}
\end{align}%
%
The above computation can be written visualized in terms of a graph as shown in
Figure~\ref{fig:mean-and-variance-of-cbf-r-diagram}.
Note that in the graph there are only two operators, the gradient and the dot
product.

\begin{figure}
\input{tex/mean-and-variance-of-cbf-r-diagram.tex}
\caption{Computation graph for higher order Lie derivative}
\label{fig:mean-and-variance-of-cbf-r-diagram}
\end{figure}


We have already shown that $\Lie_f^{(2)} h(\bfx)$ is a Gaussian process whose
mean and variance can be analytically computed. We focus our attention on
$\Lie_f^{(3)} h(\bfx)$.

%
\begin{align}
  \Lie_f^{(3)} h(\bfx) = \grad [\Lie_f^{(2)} h(\bfx)]^\top f(\bfx)
\end{align}%
%

By Lemma~\ref{lemma:differentiating-gp}, the gradient of a GP $\grad \Lie_f^{(2)}
h(\bfx)$ is also a Gaussian Process.
We again write $\grad [\Lie_f^{(2)} h(\bfx)]^\top f(\bfx)$ in a quadratic form,

%
\begin{align}
  \Lie_f^{(3)} h(\bfx)
  &=
    \begin{bmatrix}
      \grad [\Lie_f^{(2)} h(\bfx)] \\
      f(\bfx)
 \end{bmatrix}^\top
\begin{bmatrix}
  0.5 & 0 \\
  0 & 0.5
\end{bmatrix}
    \underbrace{\begin{bmatrix}
      \grad [\Lie_f^{(2)} h(\bfx)] \\
      f(\bfx)
 \end{bmatrix}}_{:= z(\bfx)}
\end{align}
%

Also let the variance of $z(\bfx)$ be $\Var(z(\bfx))$. Let the Cholesky
factorization of $\Var(z(\bfx))$ be $A(\bfx)A(\bfx)^\top := \Var(z(\bfx))$.
Then $w(\bfx) := A^{-1}(\bfx) (z(\bfx)-\E[z(\bfx)]) $ has the variance as identity:
%
\begin{align}
  \Var(w(\bfx)) := \E[w(\bfx)w(\bfx)^\top]
  = \E[ A^{-1}(\bfx) z(\bfx) z(\bfx)^\top A^{-\top}(\bfx) ]
  = A^{-1}(\bfx) \Var(z(\bfx)) A^{-\top}(\bfx) = I.
\end{align}%
%

So $\Lie_f^{(3)} h(\bfx)$ can be written in terms of $w(\bfx)$,
%
\begin{align}
  \Lie_f^{(3)} h(\bfx)
  &= w(\bfx)^\top
  \underbrace{A^\top(\bfx)
  \begin{bmatrix} 0 & 0.5 \\ 0.5 & 0 \end{bmatrix}
                                 A(\bfx)
                                 }_{\Lambda(\bfx)}
                                 w(\bfx)
                                 + 2 w(\bfx)^\top A(\bfx)\E[z(\bfx)] 
                                 + \E[z(\bfx)]^2
  \\
  &= w(\bfx)^\top \Lambda(\bfx) w(\bfx)
  + 2 w(\bfx)^\top A(\bfx)\E[z(\bfx)] 
  + \E[z(\bfx)]^2
\end{align}
%

Note that $w(\bfx)$ is a zero-mean unit variance Gaussian random vector with
independent coordinates. Next we recall a recent extension of Hansen-Wright
inequality~\cite{gotze2019concentration},

%
\begin{definition}[Orclitz norm]
  The Orclitz norm $\|X\|_{\Psi_\alpha}$ of a random variable $X$ is defined as:
  %
  \begin{align}
    \|X\|_{\Psi_\alpha} := \inf\left\{
    t \ge 0 : \E \exp\left(\frac{\|X\|^\alpha}{t^\alpha} \right) \le 2
    \right\},
  \end{align}
  %
  where $\inf \phi = \infty$.
  Note that Orclitz norm is only a norm for $\alpha > 1$ to satisfy the
  triangle inequality.
\end{definition}

%
\begin{theorem}[Concentration of Sub-$\alpha$ exponential RV \citep{gotze2019concentration}]
  \label{thm:sub-alpha-exp-rv}
  Let $X_1, \dots, X_n$ be independent random variables satisfying $\E[X_i] = 0,
  \E[X_i^2] = \sigma_i^2, \|X_i\|_{\Psi_\alpha} \le M$ for some $\alpha \in (0,
  1] \cup \{2\}$, and $A$ be a symmetric $n \times n$ matrix.

  For any $t > 0$ we
  have,
  \begin{align}
    P\left(
    \left|
    X^\top A X - \tr( \diag(\{\sigma_i^2\}_{i=1}^n) A)
    \right| \ge t
    \right)
  \le 2 \exp\left(-\frac{1}{C}
    \min\left( \frac{t^2}{M^4 \|A\|_{HS}^2},
      \left(\frac{t}{M^2 \|A\|_{op}} \right)^{\frac{\alpha}{2}}
      \right)
    \right).
    \end{align}
\end{theorem}
%

For our case, $X_i = w(\bfx)_i$ and all $\sigma_i = 1$. Also the Orclitz norm
$\|X_i\|_{\Psi_\alpha}$ for $\alpha = 2$ exists for sub-Gaussian random
variables.
Since, $w(\bfx)_i$ is Gaussian random variables, hence
$\|w(\bfx)_i\|_{\Psi_\alpha}$ exists with $\alpha = 2$.

Applying Theorem~\ref{thm:sub-alpha-exp-rv} to $w(\bfx)^\top \Lambda(\bfx)
w(\bfx)$ with $\alpha = 2$, we get,
%
\begin{align}
  P\left(\left| w(\bfx)^\top \Lambda(\bfx) w(\bfx) - \tr(\Lambda(\bfx)) \right| \ge t \right)
  \le 2 \exp\left(-\frac{1}{C}
    \min\left( \frac{t^2}{M^4 \|\Lambda(\bfx)\|_{HS}^2},
      \frac{t}{M^2 \|\Lambda(\bfx)\|_{op}}
      \right)
    \right).
\end{align}

We already know that $w(\bfx)$ being a Gaussian random vector,
%
\begin{align}
  P\left(\left| w(\bfx)^\top A(\bfx) E[z(\bfx)] \right| \ge t \right)
  \le c \exp\left(-\frac{t^2}{C} \right)
\end{align}
%

We can conclude that
$\Lie^{(3)}_f h(\bfx)$ is sub-exponential random vector,
%
\begin{align}
  P\left( \left| \Lie^{(3)}_f h(\bfx) - \E[\Lie^{(3)}_f h(\bfx)] \right| \ge t \right)
  \le C \exp\left( -\frac{t}{c} \right).
\end{align}%
% 

We have already seen that derivative of the random process with exponential
kernel does not change the the tail bounds of the random process.

For arbitrary $r \ge 2$th Lie derivative, we have
%
\begin{align}
  P\left( \left| \Lie^{(r)}_f h(\bfx)
  - \E[\Lie^{(r)}_f h(\bfx)] \right| \ge t \right)
  \le C \exp\left( -\frac{t^{\frac{2}{r-1}}}{c} \right).
\end{align}
  

==> tex/rem112.tex <==
\begin{remark}
\label{remar1!}
\rm{
Assuming  $\|\dot{x}(t_k)\|\neq0$ in Theorem~\eqref{ir5o45t!!!} is not restricting our results. Since, if the state of the system is safe and it does not change it remains safe. 

%As discussed, for consistent learning algorithm $p_k \rightarrow 1$ as $k \rightarrow \infty$. In this case as $T \rightarrow \infty$ for any $\epsilon >0$ there exist  $k_0 \in \mathbb{N}$ such that 
% \begin{align}
%     \prod_{k=k_0}^{\infty} p_k \ge 1-\epsilon.
% \end{align}
% In this case the controller $u$ renders the set $\mathcal{C}$ safe as time tends to infinity with probability at least 
%  \begin{align}
%     (1-\epsilon)\prod_{k=0}^{k_0} p_k.
% \end{align}
%
The lower bound~\eqref{lowerboun44!!22} is derived based on the independence of the events, it is not tight in general. In fact,
the chance constraint in program~\eqref{prog:CBF-CLF:unknown} can be replaced by
\begin{align}
   \mathbb{P}(\mbox{CBC}_k \ge \zeta | \bfx_k,\bfu_k, \mbox{CBC}_{k-1} \ge \zeta) \ge p_{k|k-1}, 
\end{align}
where $p_{k|k-1}$ is the lower bound of the chance constraint at $k$th triggering time provided that CBC was at least $\zeta$ in the $k-1$th triggering time, and $\mbox{CBC}_0$ is the value of CBC at time $0$. Assume the GP sample paths are sufficiently smooth such that there exist a sufficiently large $L_k$ for which the event~\eqref{eq:smoth23} occurs at all triggering time. Then the safety probability can be lower-bounded by  \begin{align}
 \prod_{k=1}^{N(T)} p_{k|k-1}.
 \end{align}
 As the controller observe more data, under BI, the posterior probability will concentrate on the true model. Thus, we can use tighter chance constraints in program~\eqref{prog:CBF-CLF:unknown}. 
 We leave these treatments for future research.
 }
 \end{remark}
